Unsupervised Domain Adaptation with Temporal-Consistent Self-Training for 3D Hand-Object Joint Reconstruction

Deep learning-solutions for hand-object 3D pose and shape estimation are now very effective when an annotated dataset is available to train them to handle the scenarios and lighting conditions they will encounter at test time. Unfortunately, this is not always the case, and one often has to resort to training them on synthetic data, which does not guarantee that they will work well in real situations. In this paper, we introduce an effective approach to addressing this challenge by exploiting 3D geometric constraints within a cycle generative adversarial network (CycleGAN) to perform domain adaptation. Furthermore, in contrast to most existing works, which fail to leverage the rich temporal information available in unlabeled real videos as a source of supervision, we propose to enforce short- and long-term temporal consistency to fine-tune the domain-adapted model in a self-supervised fashion. We will demonstrate that our approach outperforms state-of-the-art 3D hand-object joint reconstruction methods on three widely-used benchmarks and will make our code publicly available.

==> fig/cyclegan.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
	\centering
	\includegraphics[width=0.50\textwidth]{images/hand_cyc/cyclegan.pdf}
	%\vspace{-2mm}
	\caption{ Inspired by the recent research on style transfer and domain adaption with generative adversary network, \ie, CycleGAN, we proposed a cross-domain image-to-image translation network, which does not need one-to-one pairs for training. Since there are generally no paired ground-truth images for supervising the domain transfer. CycleGAN is adopted as our backbone to convert images back and forth between the realistic image domain and the rendered image domain. To better preserve geometry information during domain translation, we introduce a shape consistency loss function as an additional constraint to train the generative model. 
}
	\label{fig:hand_model2}
	%\vspace{-2mm}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	


==> fig/hand_model.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
	\centering
	\includegraphics[width=0.90\textwidth]{images/hand_cyc/hand_model.pdf}
	%\vspace{-2mm}
	\caption{Overall architecture of the proposed joint 3D hand-object reconstruction framework with a geometry-preserved domain transfer generative network to bridge the domain gap between synthetic and realistic image domain. The whole architecture mainly consists of two part: a 3D pose based CycleGAN to translate labeled synthetic data into realistic-style data, and a baseline model~\cite{Hasson19} is adopted to output 3D reconstruction results. The baseline model has an encoder to capture visual information from input images, and a hand decoder and a object decoder are leveraged to estimate the pose and shape of hands and objects, respectively.
}
	\label{fig:hand_model3}
	%\vspace{-2mm}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	


==> fig/result_synthetic.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
	\centering
	\includegraphics[width=0.75\textwidth]{images/hand_example/result_synthetic.pdf}
	%\vspace{-1mm}
	\caption{Qualitative results of our proposed model tested on synthetic domain data, \ie,~\emph{ObMan Dataset}.}
	\label{fig:result_synthetic2}
	%\vspace{-1mm}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%		


==> fig/result_synthetic_copy.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
	\centering
	\includegraphics[width=0.75\textwidth]{images/hand_example/result_synthetic.pdf}
	%\vspace{-1mm}
	\caption{Qualitative results of our proposed model tested on synthetic domain data, \ie,~\emph{ObMan Dataset}.}
	\label{fig:result_synthetic2}
	%\vspace{-1mm}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%		


==> table/crowd.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US


\begin{table}[!t]
	\centering
	\caption{Performance comparison of our proposed model (3rd iteration), the baseline model, and UDA state-of-the-art methods on {\bf JHU-CROWD++}~\cite{Sindagi20b} dataset among rain, fog and snow weather conditions respectively. The best result is denoted in bold.}
	\resizebox{0.995\linewidth}{!}{
		\begin{tabular}{lcccccc}
			\toprule
      \multirow{2}{*}{Methods}  &\multicolumn{2}{c}{ Rain} &\multicolumn{2}{c}{Fog} &\multicolumn{2}{c}{ Snow}\\
      \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}&\tabincell{c}{MAE} & \tabincell{c}{RMSE}  & \tabincell{c}{MAE} & \tabincell{c}{RMSE}  & \tabincell{c}{MAE} & \tabincell{c}{RMSE} \\  \midrule
			No DA                    & 168.6 & 236.2   & 120.4 & 168.3 & 192.6 & 218.6\\
			UDA~w/~Cycada~\cite{Hoffman18}     & 153.2 & 210.2  & 106.9 & 141.8 & 184.1 & 196.7\\ 
			UDA~w/~FDA~\cite{Yang20b}     &167.3 & 233.8 &  117.4 & 162.9  & 190.8 & 219.2 \\
			UDA~w/~DANN~\cite{Tzeng17}    &  &   &  &  &  & \\
			UDA~w/~ADDA~\cite{Ganin15}     &  &  &  &  &  & \\ \midrule
			\oursC                  & 151.8 & 206.3 & 103.5 & 133.6  & 181.2 & 190.5\\  
			\oursT                  &  \textbf{150.3} & \textbf{200.5} & \textbf{101.7} & \textbf{128.9}  & \textbf{178.4} & \textbf{188.2} \\
			\bottomrule	   
	\end{tabular}}	
	%\vspace{+1mm}
	\label{tab:performance_crowd}
	%\vspace{-3mm}		
\end{table}
